Software Model-Checking as Cyclic-Proof Search

This paper shows that a variety of software model-checking algorithms can be seen as proof-search strategies for a non-standard proof system, known as a cyclic proof system. Our use of the cyclic proof system as a logical foundation of software model checking enables us to compare different algorithms, to reconstruct well-known algorithms from a few simple principles, and to obtain soundness proofs of algorithms for free. Among others, we show the significance of a heuristics based on a notion that we call maximal conservativity; this explains the cores of important algorithms such as property-directed reachability (PDR) and reveals a surprising connection to an efficient solver of games over infinite graphs that was not regarded as a kind of PDR.

==> appx-k-ind.tex <==
\section{On the Cyclic Proof Corresponding to $k$-Induction}
In terms of cyclic-proof search, this approach can be explained as follows.
Let \( \Theta(y) \) be \( \exists x. \Cum{k}(\alpha)(x) \wedge \tau(x,y) \) and suppose \( \Theta(x) \models \alpha(x) \).
We have \( \varphi_k(x) \Rightarrow \Cum{k}(\alpha)(x) \) as a consequence of bounded safety.
Therefore
\begin{align*}
    \varphi_{k+1}(x\hu{y?})
    &~~\Leftrightarrow~~
    \exists x. \varphi_k(x) \wedge \tau(x,y)
    \\
    &~~\Rightarrow~~
    \exists x. \Cum{k}(\alpha)(x) \wedge \tau(x,y)
    & (\Leftrightarrow \Theta(y))
    \\
    &~~\Leftrightarrow~~
    \alpha(y) \wedge \exists x. \Cum{k}(\alpha)(x) \wedge \tau(x,y)
    & \qquad(\mbox{since \( \Theta(y) \models \alpha(y) \)})
    \\
    &~~\Rightarrow~~
    \Cum{k+1}(\alpha)(y)
\end{align*}
and thus
\begin{equation*}
    \exists x. \Theta(x) \wedge \tau(x,y)
    ~~\Leftrightarrow~~
    \exists x. \alpha(x) \wedge \Theta(x) \wedge \tau(x,y)
    ~~\Rightarrow~~
    \exists x. \Cum{k+1}(\alpha)(x) \wedge \tau(x,y)
\end{equation*}
of which the last formula implies \( \Theta(y) \) since \( \Cum{k+1}(\alpha)(x) \Rightarrow \Cum{k}(\alpha)(x) \).
Then, by using \textsc{(Cut)} rule,
\begin{equation*}
    \infer{
        \varphi_{k+1}(x) \vdash (\nu P)(x)
    }{
        \varphi_{k+1}(x) \models \Theta(x)
        &&
        \hspace{-50pt}
        \infer[\textsc{(SE)}]{
            \Theta(x) \vdash (\nu P)(x)
        }{
            \infer{
                \exists x. \Theta(x) \wedge \tau(x,y) \vdash (\nu P)(y)
            }{
                \exists x. \Theta(x) \wedge \tau(x,y) \models \Theta(y)
                &&
                \Theta(x) \vdash (\nu P)(x)
            }
            &&
            \Theta(x) \models \alpha(x)
        }
    }
\end{equation*}
One can complete the proof by making a link from the open sequent \( \Theta(x) \vdash (\nu P)(x) \) to an appropriate ancestor.


==> appx-mc-algo.tex <==
\section{An Algorithm Computing a Maximally Conservative Interpolant}
\begin{figure}[t]
    \centering
    \begin{enumerate}
        \item \( k \leftarrow n-1 \)
        \item If an interpolant of \( \varphi_k, \varphi_{k+1}, \dots, \varphi_n \) exists:
        \begin{enumerate}
            \item Let \( \psi_k, \psi_{k+1}, \dots, \psi_n \) be an interpolant.
            \item Return \( \top, \dots, \top, \psi_{k}, \psi_{k+1}, \dots, \psi_n \).
        \end{enumerate}
        \item If \( k = 1 \), return \texttt{No} \texttt{//} No interpolant exists
        \item \( k \leftarrow k-1 \); goto 2
    \end{enumerate}
    \caption{Algorithm to compute a maximally conservative interpolant for \( \vec{\varphi} = \varphi_1, \dots, \varphi_n \).  For simplicity, we assume that \( \varphi_{i-1} \Rightarrow \varphi_i \) holds for every \( i \) but the last one \( i=n \), which every instance appearing in McMillan's algorithm satisfies.}
    \label{fig:algorithm-for-mc-interpolant}
\end{figure}

\autoref{fig:algorithm-for-mc-interpolant} gives an algorithm, which iteratively computes an interpolation of \( \varphi_k, \varphi_{k+1}, \dots, \varphi_n \) for \( k = n-1, n-2, \dots, 1 \) until the algorithm finds it.



==> dualimpact.tex <==
\subsection{Dual sequent and dual \impact{}}
\label{sec:dualimpact}
As we have seen in Section~\ref{sec:pre}\tk{pre?}, a linear CHC system has a characterization by least fixed-points.
Concretely, a linear CHC system with \( n \) predicate variables
\begin{equation*}
    \iota(x) \Rightarrow P_1(x),
    \qquad
    P_i(x) \wedge \tau_{i,j}(x,y) \Rightarrow P_j(y)
    \quad(i,j = 1,\dots,n),
    \qquad
    P_n(x) \Rightarrow \alpha(x),
\end{equation*}
(where \( P_1 \) corresponds to the entry point and \( P_n \) the assertion)
is satisfiable if and only if \( (\mu P_n)(x) \vdash \alpha(x) \) where \( \mu P_i \), \( i = 1,\dots,n \), is the least solution of
\begin{align*}
    \iota(y) \vee \bigvee_{i=1,\dots,n} \left( \exists x. (\mu P_i)(x) \wedge \tau_{i,1}(x,y) \right) &\qquad\Leftrightarrow\qquad (\mu P_1)(y)
    \\
    \bigvee_{i=1,\dots,n} \left( \exists x. (\mu P_i)(x) \wedge \tau_{i,j}(x,y) \right) &\qquad\Leftrightarrow\qquad (\mu P_j)(y)
    & (j = 2,\dots,n).
\end{align*}

The goal-oriented proof search for \( (\mu P_n)(x) \vdash \alpha(x) \) corresponds to a variant of \impact{}, applied to the \emph{dual system} obtained by reverting the arrows of the control flow graph.
\begin{equation*}
    \dfrac{
        (\mu P_1)(x) \vdash \varphi_1(x)
        \quad\dots\quad
        (\mu P_n)(x) \vdash \varphi_n(x)
        \qquad
        \bigvee_{i=1,\dots,n} \left( \exists x. \varphi_i(x) \wedge \tau_{i,j}(x,y) \right) \models \varphi'_j(y)
    }{
        (\mu P_j)(y) \vdash \varphi'_j(y)
    }
\end{equation*}


\ifverylong
\subsection{Forward proof search}
\tk{todo}



have explained PDR as a goal-oriented proof search strategy for the dual formulation of the safety verification, namely \(\iota(x) \vdash (\nu X. \lambda x. \alpha(x) \wedge \forall y. \tau(x,y) \Rightarrow X(y))(x)\).
This section aims to provide another viewpoint; PDR can be seen as a proof search of the standard safety judgement \((\mu X.\lambda x. \iota(x) \vee \exists y. X(y) \wedge \tau(y,x))(x) \vdash \alpha(x)\).

A state of the proof search procedure can be represented as a partial proof with annotations.
Some judgements \((\mu X)(x) \vdash \varphi(x)\) in a partial proof are annotated with formulas \(\psi(x)\), written \((\mu X)(x) \vdash \varphi(x) \upharpoonright \psi_1(x), \dots \psi_n(x)\), meaning that we would like to strengthen the current conclusion \((\mu X)(x) \vdash \varphi(x)\) to \((\mu X)(x) \vdash \varphi(x) \wedge \psi_1(x) \wedge \dots \psi_n(x)\).
Unlike the goal-oriented proof search studied in previous sections, the partial proofs appearing in this section are always valid although the conclusion is weaker than that we expect.

The proof search process can be seen as a rewriting process of partial proofs, strengthening the partial proof while keeping its validity.
Assume that we have obtained a partial proof \(\Pi\) of height \(k\) (i.e.~we have checked \(k\)-bounded safety).
Then we try to make the partial proof a proof, by closing the open leaf.
If it fails, we construct the following valid partial proof of height \(k+1\) by adding a new node to the root:
\begin{equation*}
    \infer{
        (\mu X)(y) \vdash \top
    }{
        \infer{(\mu X)(x) \vdash \varphi(x)}{\Pi}
        &&
        \iota(y) \vee \exists x. (\varphi(x) \wedge \tau(x,y)) \vDash \top
    }
\end{equation*}
Note that this is valid.
Unfortunately the conclusion \((\mu X)(x) \vdash \top\) does not suffice to show the safety.
So we would like to strengthen the proof.

Assume that the current conclusion is \( (\mu X)(x) \vdash \varphi(x) \upharpoonright \vec{\theta}(x)\) and \( \varphi(x) \nvDash \alpha(x) \).
Let \( \psi(x) \nvDash \varphi(x) \wedge \neg \alpha(x) \).
Then we change the conclusion to \( (\mu X)(x) \vdash \varphi(x) \upharpoonright \vec{\theta}(x), \neg \psi(x) \).

If a requirement \( \psi(x) \) for a judgement in the partial proof has already fulfilled, i.e.~the judgement is \( (\mu X)(x) \vdash \varphi(x) \upharpoonright \dots, \psi(x), \dots \) with \( \varphi(x) \vDash \psi(x) \), we simply remove \( \psi(x) \) from the requirement list.

Assume that the partial proof contains the following part:
\begin{equation*}
    \infer{
        \infer{\vdots}{(\mu X)(x) \vdash \varphi(x) \upharpoonright \dots, \psi(x), \dots}
    }{
        \infer{(\mu X)(x) \vdash \varphi'(x) \upharpoonright \vec{\theta}(x)}{\vdots}
        &&
        \varphi'(x) \wedge \tau(x,y) \vDash \varphi(x)
    }
\end{equation*}
and \( \psi'(x) \) is a sufficient condition for the premise that ensures the conclusion is stronger than \(\psi(x)\), i.e.~\(\psi'(x) \wedge \tau(x,y) \models \psi(x)\), then this part can be rewritten to
\begin{equation*}
    \infer{
        \infer{\vdots}{(\mu X)(x) \vdash \varphi(x) \upharpoonright \dots, \psi(x), \dots}
    }{
        \infer{(\mu X)(x) \vdash \varphi'(x) \upharpoonright \vec{\theta}(x), \psi'(x)}{\vdots}
        &&
        \varphi'(x) \wedge \tau(x,y) \vDash \varphi(x)
    }
\end{equation*}

We can also annotate the proof by under-approximations of \((\mu X)(x)\) as \( \varpi(x) \downharpoonleft (\mu X)(x) \vdash \varphi(x) \), meaning that \( \varphi(x) \models (\mu X)(x) \).
This information can be propagated top-down: if the current partial proof is
\begin{equation*}
    \infer{
        \infer{\vdots}{(\mu X)(x) \vdash \varphi(x) \upharpoonright \vec{\theta}(x)}
    }{
        \infer{\varpi'(x) \downharpoonleft (\mu X)(x) \vdash \varphi'(x) \upharpoonright \vec{\theta}'(x)}{\vdots}
        &&
        \varphi'(x) \wedge \tau(x,y) \vDash \varphi(x)
    }
\end{equation*}
and \( \varpi(x) \models \varpi'(x) \wedge \tau(x,y) \), then the partial proof can be rewritten to
\begin{equation*}
    \infer{
        \infer{\vdots}{\varpi(x) \downharpoonleft (\mu X)(x) \vdash \varphi(x) \upharpoonright \vec{\theta}(x)}
    }{
        \infer{\varpi'(x) \downharpoonleft (\mu X)(x) \vdash \varphi'(x) \upharpoonright \vec{\theta}'(x)}{\vdots}
        &&
        \varphi'(x) \wedge \tau(x,y) \vDash \varphi(x)
    }
\end{equation*}
However, unrestricted use of this rule is inefficient.
So this top-down propagation is allowed only if \(\omega(x)\) refutes a requirement, i.e.~there exists \(\theta_i \in \vec{\theta}\) such that \(\omega(x) \nVdash \theta_i(x)\) (that implies \((\mu X)(x) \nvDash \theta_i(x)\)).
\fi


==> hbpdr.tex <==
\subsection{HB-PDR}
\label{sec:real:pdr}
\paragraph{Definition of PDR.}
Our description of the algorithm is based on the abstract transition system given by Hoder and Bj{\o}rner~\cite{Hoder2012}.
A \emph{configuration} is of the form \( (c_k \dots c_n \parallel F_0 F_1 \dots F_n) \), consisting of two sequences of \emph{(candidate) counterexamples} \( c_i \in \mathcal{S} \) and \emph{frames} \( F_i \),%
    \footnote{We do not use metavariables \( \varphi \) and \( \psi \) for frames, because a frame does not precisely correspond to a cut-formula.  See a discussion below.}
which are formulas denoting unary predicates.
We call \( c_i \) (resp.~\( F_i \)) the counterexample (resp.~the frame) at \emph{level} \( i \).
Note that counterexamples are associated to only higher levels and that the counterexample sequence can be empty \( \epsilon \).
Intuitively a frame \( F_i \) at level \( i \) denotes an over-approximation of states of distance \( \le i \) and \( c_i \) together with \( c_{i+1} \dots c_n \) is a witness of unsafety of \( F_i \) with bound \( (n-i) \), i.e.~\( F_i(c_i) \) and \( \bigwedge_{j=i}^{n-1} \tau(c_j, c_{j+1}) \wedge \neg \alpha(c_n) \).
Formally each configuration \( (c_k \dots c_n \parallel F_0 \dots F_n) \) must satisfy (a)~\( F_0 = \iota \), (b)~\( F_i(x) \vee \mathcal{F}(F_i)(x) \models F_{i+1}(x) \) for every \( 0 \le i \le n \),%
    \footnote{\( \mathcal{F} \) is the predicate transformer given by \( \mathcal{F}(F)(y) := \iota(y) \vee (\exists x. F(x) \wedge \tau(x,y)) \).}
(c) \( F_{i}(x) \models \alpha(x) \) for every \( 0 \le i < n \), (d)~\( \models F_i(c_i) \) for every \( k \le i \le n \), and (e)~\( \models \bigwedge_{i=k}^{n-1} \tau(c_i, c_{i+1}) \wedge \neg \alpha(c_n) \).

A configuration \( (\vec{c} \parallel F_0 \dots F_n) \) is \emph{boundedly safe} if \( F_n(x) \models \alpha(x) \).
Note that this implies \( \vec{c} = \epsilon \).
If the configuration is boundedly safe, \( F_i \) is safe with bound \( (n-i) \) for every \( 0 \le i \le n \) and, in particular, \( F_0 = \iota \) is safe with bound \( n \).
To emphasize a configuration is boundedly safe, we write it as \( (\epsilon \parallel F_0 \dots F_n~\checkmark) \).

The transition rules are given in \autoref{fig:PDR}.
The rule \textsc{(Unfold)} is applicable when \( F_0 = \iota \) has been confirmed safe with bound \( n \).
This rule starts to check if \( \iota \) is safe with bound \( (n+1) \), by extending the frame by \( \top \).
\textsc{(Candidate)} is applicable when a state \( c_n \) satisfying \( F_n \) violates the assertion \( \alpha \) and starts to check if the bad state \( c_n \) is \( n \)-step reachable from \( \iota \).
The candidate counterexample is propagated backward by \textsc{(Decide)} rule.
If \textsc{(Decide)} is not applicable, the candidate is spurious, i.e.~it was introduced by the approximation at this level.
Then \textsc{(Conflict)} refines the approximation, strengthening \( F_k \) so that it does not contain the spurious counterexample \( c_k \) (i.e.~\( G(x) \models x \neq c_k \)).
%
\begin{figure}[t]
    %\hu{$\psi$ should be replaced by $G$?}
    %\tk{Right.  Thanks.}
    \begin{gather*}
        \infer[\textsc{(Unfold)}]{
            (\epsilon \parallel F_0 \dots F_n ~\checkmark) \longrightarrow (\epsilon \parallel F_0 \dots F_n \top)
        }{}
        \\[5pt]
        \infer[\textsc{(Candidate)}]{
            (\epsilon \parallel F_0 \dots F_n) \longrightarrow (c \parallel F_0 \dots F_n)
        }{
            \models F_n(c) \wedge \neg \alpha(c)
        }
        \\[5pt]
        \infer[\textsc{(Decide)}]{
            (c_k\,\dots\,c_n \parallel F_0 \dots F_n) \longrightarrow (c' c_k \dots c_n \parallel F_0 \dots F_n)
        }{
            \models F_{k-1}(c') \wedge \tau(c', c_k)
        }
        \\[5pt]
        \infer[\textsc{(Conflict)}]{
            (c_k \dots c_n \parallel F_0 \dots F_n)
            \longrightarrow
            (c_{k+1} \dots c_n \parallel F_0 \dots F_{k-1} (F_{k} \wedge \psi) F_{k+1} \dots F_n)    
        }{
            \mathcal{F}(F_{k-1})(x) \vee F_{k-1}(x) \models G(x)
            \qquad
            G(x) \models x \neq c_k
        }
    \end{gather*}
    \vspace{-20pt}
    \caption{The transition rules for PDR.}
    \label{fig:PDR}
\end{figure}

The initial configuration is \( (\epsilon \parallel \iota) \).
If it reaches \( (\epsilon \parallel F_0 \dots F_n ~\checkmark) \) with \( F_n(x) \models F_{n-1}(x) \), then the program is safe and an invariant is \( F_n \).
If it reaches \( (c_0 \dots c_n \parallel F_0 \dots F_n) \) with a counterexample at level \( 0 \), the program is unsafe.


\paragraph{PDR vs.~\impact{} with MC interpolants.}


The key observation is that \( F_i \) is unchanged if it is safe with bound \( (n-i+1) \): this is true because no counterexample reaches level \( i \).
In other words, PDR does not change a frame \emph{unless} its update is inevitable to make the frame sequence boundedly safe~\cite[Section~III.E]{Een2011}.
This property is actually the maximum conservativity.

Let us discuss the relationship in more detail.
A state of \impact{}, or a partial proof as in \autoref{fig:impact-partial-proof}, satisfies most conditions for a frame sequence of PDR, but \( \varphi_i(x) \models \varphi_{i+1}(x) \) is not necessarily true in \impact{}.
To fill the gap, the frame sequence corresponding to \autoref{fig:impact-partial-proof} is defined by
\begin{equation*}
    \textstyle
    \mathit{frames}(\varphi_0 \dots \varphi_n)
    ~~:=~~
    \varphi_0 (\bigvee_{i=0}^{1} \varphi_i) \dots (\bigvee_{i=0}^{n} \varphi_i)
\end{equation*}
If the cut-formulas \( \varphi_i \) in \autoref{fig:impact-partial-proof} is updated to \( \varphi_i' \) by using a maximally conservative interpolant, we write
\(
    (\epsilon \parallel \mathit{frames}(\varphi_0 \dots \varphi_n)) \stackrel{\textsc{(MC)}}{\rightsquigarrow} (\epsilon \parallel \mathit{frames}(\varphi'_0 \dots \varphi'_n))
\).%
    \footnote{%
        We note that \( \stackrel{\textsc{(MC)}}{\rightsquigarrow} \) depends only on the frames \( \mathit{frames}(\varphi_0 \dots \varphi_n) \) and independent of the choice of the cut formulas \( (\varphi_i)_{i = 0, \dots, n} \).
        That means, if \( \mathit{frames}(\varphi_0 \dots \varphi_n) = \mathit{frames}(\psi_0 \dots \psi_n) \), then \( (\psi_i)_{i=0,\dots,n} \) can be refined to \( (\psi'_i)_{i=0,\dots,n} \) which satisfies \( \mathit{frames}(\varphi'_0 \dots \varphi'_n) = \mathit{frames}(\psi_0' \dots \psi_n') \).
        Hence Theorem~\ref{thm:PDR-MC} says that \( \mathit{frames} \) is a functional bisimulation from \impact{} with MC interpolation to PDR in a certain sense.}
% To formalize the claim, we introduce a rewriting rule \( \stackrel{\textsc{(MC)}}{\rightsquigarrow} \) based on maximally conservative interpolation. 
% \hu{\textsc{(MC)} and the notion of maximally consistent not explained? maximally conservative?}
% : the sequence \( \top, \psi_1(x_1), \dots, \psi_{n+1}(x_{n+1}), \bot \) of formulas is an interpolant of \( \iota(x_0) \wedge \tau(x_0, x_1), \tau(x_1, x_2), \dots, \tau(x_{n}, x_{n+1}), \neg \alpha(x_n) \).
%
% The next theorem gives a complete characterization of interpolants generated by PDR.
% Simply they are maximally conservative.
%

\begin{remark}
    PDR given in this subsection somewhat differs from that by Hoder and Bj{\o}rner~\cite{Hoder2012}.
    Most differences are minor ones, except for the difference of the condition for \( \psi \) in \textsc{(Conflict)} and the lack of \textsc{(Induction)}.
    The difference on \textsc{(Conflict)} is the topic of \autoref{sec:hb-pdr}.
    \textsc{(Induction)} is discussed in \autoref{rem:pdr-induction}.
    %
    \qed
\end{remark}

\begin{remark}
    \label{rem:pdr_interpolants}
    We discuss a limitation of the logical characterization of PDR.
    The above-mentioned consequence of Theorem~\ref{thm:PDR-MC} is that PDR coincides with \impact{} with MC interpolation if \emph{the backend interpolating theorem prover returns an interpolant completely nondeterministically}.
    This assumption is not true in practice.
    It may be the case that the efficiency of PDR essentially relies on some properties of typical or existing provers and some details of PDR, which cannot be captured by Theorem~\ref{thm:PDR-MC}.
    For example, Cimatti and Griggio~\cite[Section~5]{Cimatti2012} pointed out that an interpolant obtained by PDR tends to be a conjunction of many simple formulas and discussed the significance of this property.
    %
    \qed
\end{remark}

\begin{remark}\label{rem:pdr-induction}
    PDR has \textsc{(Induction)} rule: for a subformula \( G \) of a frame, if \( \mathcal{F}(F_i \wedge G)(x) \models G(x) \), then \( (\vec{c} \parallel F_0 \dots F_n) \to (\vec{c} \parallel (F_0 \wedge G) \dots (F_{i+1} \wedge G) F_{i+1}\hu{F_{i+2}?} \dots F_n) \).
    Although \impact{} with MC interpolants does not have a corresponding rule, \textsc{(Induction)} can be seen as a meta-theorem transforming a partial proof to another partial proof.
    %
    \qed
\end{remark}

\subsection{PDR in the Hoder-Bj{\o}rner style}\label{sec:hb-pdr}
The \textsc{(Conflict)} rule studied in the previous subsection differs from that in Hoder and Bj{\o}rner~\cite{Hoder2012}.
\tkchanged{Here is the rule of Hoder and Bj{\o}rner~\cite{Hoder2012}:
\begin{equation*}
    \infer[\textsc{(Conflict')}.]{
        (c_k \vec{c} \parallel \vec{F})
        \longrightarrow
        (\vec{c} \parallel (F_0 \wedge G) \dots (F_{k} \wedge G) F_{k+1} \dots F_n)    
    }{
        \mathit{len}(\vec{c}) = n-k 
        &&
        \mathcal{F}(F_{k-1})(x) \models G(x)
        &&
        G(x) \models x \neq c_k
    }
\end{equation*}
}
%The rule of Hoder and Bj{\o}rner~\cite{Hoder2012} is shown in \autoref{fig:HB-PDR}.
Let us call the PDR with \textsc{(Conflict')} rule \emph{HB-PDR} in order to avoid confusion with PDR in the previous subsection.
This subsection investigates a declarative variant of the interpolation by HB-PDR.

% \begin{figure}[t]
%     \tk{The rule of this figure was inlined.}
%     \begin{equation*}
%         \infer[\textsc{(Conflict')}]{
%             (c_k \vec{c} \parallel \vec{F})
%             \longrightarrow
%             (\vec{c} \parallel (F_0 \wedge G) \dots (F_{k} \wedge G) F_{k+1} \dots F_n)    
%         }{
%             \mathit{len}(\vec{c}) = n-k 
%             &&
%             \mathcal{F}(F_{k-1})(x) \models G(x)
%             &&
%             G(x) \models x \neq c_k
%         }
%     \end{equation*}
%     \caption{The conflict rule in Hoder and Bj{\o}rner~\cite{Hoder2012}.}
%     \label{fig:HB-PDR}
% \end{figure}

There is a significant difference.
\textsc{(Conflict')} may strengthen boundedly safe frames whereas \textsc{(Conflict)} never changes such frames.
\textsc{(Conflict)} rule can be seen as a special case of \textsc{(Conflict')} rule where \( G \) additionally satisfies \( F_{k-1}(y) \Rightarrow G(y) \).
Hence \textsc{(Conflict')} rule makes more configurations
%states\hu{configurations?}\tk{Yes.  Thanks.}
reachable.

Perhaps surprisingly \textsc{(Conflict')} rule is closely related to \( k \)-induction (see \autoref{sec:k-induction}).
% Recall that the key idea of the \( k \)-induction for proving \( P \) is to use another property saying that \( P \) is satisfied in \( k \) consecutive steps.
% We define \( k\textit{-Ind}(P) \) by
% \begin{equation*}
%     k\textit{-Ind}(P)(x_k)
%     \quad:\Leftrightarrow\quad
%     \exists x_1 \dots x_{k-1}. \bigwedge_{i=1,\dots,k} P(x_i) \wedge \bigwedge_{i=2,\dots,k} \Big(\iota(x_i) \vee \tau(x_{i-1}, x_i) \Big).
% \end{equation*}
% Hence \( k\textit{-Ind}(P)(x_k) \) holds if either (1) there exists a transition sequence \( x_1, \dots, x_{k-1}, x_k \) consisting of \( k \) states satisfying \( P \) or (2) there exists a transition sequence \( x_j, x_{j+1}, \dots, x_{k-1}, x_k \) (\( 1 < j \le k \)) consisting of states satisfying \( P \) where \( x_j \) is an initial state.\footnote{Here we implicitly assume that \( \iota \) is not empty.}
% Obviously \( k\textit{-Ind}(P) \Rightarrow P \), i.e.~\( k\textit{-Ind}(P) \) is stronger than \( P \).
%
We introduce a rule that strengthen \( F_\ell \) to (an over-approximation of) its \( k \)-th cumulation \( \Cum{k}(F_k) \):
\begin{equation*}
    \infer[\textsc{(\( k \)-Cum at \( \ell \))}.]{
        (\vec{c} \parallel F_0 \dots F_n) \longrightarrow
        (\vec{c} \parallel (F_0 \wedge G) \dots (F_{\ell+1} \wedge G) F_{\ell+2} \dots F_n)
    }{
        \Cum{k}(F_{\ell})(x) \models G(x)
        &&
        \mathcal{F}(F_\ell \wedge G)(x) \models G(x)
    }
\end{equation*}
For \( k = \infty \), \( \textsc{($k$-Cum at $\ell$)} \) is the union of \( \textsc{($m$-Cum at $\ell$)} \) for every \( m < \infty \).

The next theorem says that the refinement process of HB-PDR can be over- and under-approximated by \textsc{($k$-Cum at $\ell$)} followed by \textsc{(MC)}. 
%
We are not sure whether \( (2) \) is computable, but \( (1) \) and \( (3) \) are computable provided that \( k' \) and \( k \) are given.
We propose \( (1) \) and \( (3) \) as declarative alternatives of HB-PDR.
\begin{theorem}
    Let \( (\epsilon \parallel F_0 \dots F_n \top) \) be a configuration in HB-PDR.
    Let \( \ell \) be the maximum level of boundedly safe frames, \( k \) be the number of counterexamples of \( F_{\ell + 1} \) and \( k' \) be the number of total counterexamples in \( F_{\ell+1} \dots F_{n} \).
    Then \( (1) \Rightarrow (2) \Rightarrow (3) \) where
    \begin{enumerate}
        \item \( (\epsilon \parallel F_0 \dots F_n \top) \xrightarrow{\textsc{(\( k \)-Cum at \( \ell \))}} \stackrel{\textsc{(MC)}}{\longrightarrow} (\epsilon \parallel F'_0 \dots F'_{n+1}) \).
        \item \( (\epsilon \parallel F_0 \dots F_n \top) \longrightarrow^* (\epsilon \parallel F'_0 \dots F'_{n+1}~\checkmark) \) in HB-PDR.
        \item \( (\epsilon \parallel F_0 \dots F_n \top) \xrightarrow{\textsc{(\( k' \)-Cum at \( \ell \))}} \stackrel{\textsc{(MC)}}{\longrightarrow} (\epsilon \parallel F'_0 \dots F'_{n+1}) \).
    \end{enumerate}
    Furthermore \( k' \) in \( (3) \) can also be bounded by the number of \textsc{(Conflit')} rule used in the rewriting sequence of \( (2) \).
    %
    \qed
\end{theorem}


==> note.tex <==
Consider the following system:
\begin{align*}
    (x=0) &\Rightarrow P(x) \\
    P(x) \wedge (y=x+1) &\Rightarrow P(y) \\
    P(x) &\Rightarrow (x \le 5). 
\end{align*}
Then the predicate transformer \( \mathcal{F} \) is:
\begin{equation}
    \mathcal{F}(P)(x) := (x=0) \vee \exists y. P(y) \wedge (x=y+1).
\end{equation}

% One can prove by using the PDR algorithm that this system is safe.
% \begin{align*}
%     \textit{Init} & \Longrightarrow \epsilon \parallel [F_1 = (x=1)] \\
%     \textit{Unfold} & \Longrightarrow \epsilon \parallel [F_1 = (x=1), F_2 = \top] \\
%     \textit{Candidate} & \Longrightarrow [c_2 = (x=4)] \parallel [F_1 = (x=1), F_2 = \top] \\
%     & \qquad\qquad\qquad \mbox{(interpolation \( \psi_2 = (x = 2) \))} \\
%     \textit{Conflict} & \Longrightarrow \epsilon \parallel [F_1 = \bot, F_2 = (x = 2)].
% \end{align*}
% Note:
% \begin{itemize}
%     \item The final frame is safe because \( F_1 = \bot \) and thus the set of reachable states is the empty set.
%     \item The problematic rule is \emph{Conflict}: It strengthen all the frames before the focused point, but it should not do.
%     \item If the \emph{Conflict} rule only change the focused frame, then the invariant \( F_i \models F_{i+1} \) would be broken (as it is not always the case that \( F_i \models \varphi \).
%     \item There is an easy fix: Replace the condition for the interpolant \( \varphi \) from
%     \begin{equation*}
%         [F_{i-1}(x) \wedge T(x,y) \models \varphi(y)] \& [\varphi(x) \models \neg c_{i}(x)]
%     \end{equation*}
%     to
%     \begin{equation*}
%         [F_{i}(x) \wedge T(x,y) \models \varphi(y)] \& [F_i(x) \models \varphi(x)] \& [\varphi(x) \models \neg c_{i}(x)].
%     \end{equation*}
%     Then \( F_j \models \varphi \) for every \( j < i \) and thus we do not need to strengthen these frames.
% \end{itemize}

One can also construct an example of a frame which does not satisfies the required invariant:
\begin{align*}
    \textit{Init} & \Longrightarrow \epsilon \parallel [F_0 = (x=0)] \\
    \textit{Unfold} & \Longrightarrow \epsilon \parallel [F_0 = (x=0), F_1 = \top] \\
    \textit{Candidate} & \Longrightarrow [c_1 = (x=100)] \parallel [F_0 = (x=0), F_1 = \top] \\
    & \qquad\qquad\qquad \mbox{(interpolation \( \psi_1 = (x\le 1 \vee x=3) \))} \\
    \textit{Conflict} & \Longrightarrow \epsilon \parallel [F_0 = (x=0), F_1 = (x \le 1 \vee x=3)] \\
    \textit{Unfold} & \Longrightarrow \epsilon \parallel [F_0 = (x=0), F_1 = (x \le 1 \vee x=3), F_2 = \top] \\
    \textit{Candidate} & \Longrightarrow [c_2 = (x=100)] \parallel [F_0 = (x=0), F_1 = (x \le 1 \vee x=3), F_2 = \top] \\
    & \qquad\qquad\qquad \mbox{(interpolation \( \psi_2 = (x\le 4) \))} \\
    \textit{Conflict} & \Longrightarrow \epsilon \parallel [F_0 = (x=0), F_1 = (x \le 1 \vee x=3), F_2 = (x \le 4)] \\
    \textit{Unfold} & \Longrightarrow \epsilon \parallel [F_0 = (x=0), F_1 = (x \le 1 \vee x=3), F_2 = (x \le 2 \vee x = 4), F_3 = \top] \\
    \textit{Candidate} & \Longrightarrow [c_3 = (x=100)] \parallel [F_0 = (x=0), F_1 = (x \le 1 \vee x=3), F_2 = (x \le 2 \vee x = 4), F_3 = \top] \\
    & \qquad\qquad\qquad \mbox{(interpolation \( \psi_3 = (x \le 3 \vee x = 5) \))} \\
    \textit{Conflict} & \Longrightarrow \epsilon \parallel [F_0 = (x=0), F_1 = (x\le 1 \vee x=3), F_2 = (x\le 2), F_3 = (x \le 3 \vee x = 5)].
\end{align*}
Here \( \psi_3 \) is an interpolation because
\begin{align*}
    \mathcal{F}(F_2)(x)
    &~~=~~
    (x=0) \vee \exists y. F_2(y) \wedge (x=y+1)
    \\
    &~~\Leftrightarrow~~
    (x=0) \vee \exists y. (y \in \{ 0,1,2,4 \}) \wedge (x=y+1)
    \\
    &~~\Leftrightarrow~~
    (x=0) \vee (x \in \{ 1,2,3,5 \})
    \\
    &~~\Leftrightarrow~~
    (x \le 3 \vee x = 5).
\end{align*}
Note:
\begin{itemize}
    \item The final frame does NOT satisfies the invariant: \( F_2 \) does not cover the next step of \( F_1 \), i.e.~\( (x=2) \nVdash F_2 \).
\end{itemize}


==> pre.tex <==
\subsection{The duality of the reachability problem}
The \emph{reachability problem} asks, given a graph \( (S,R) \) and two sets \( I, B \subseteq S \) of nodes of \( S \), whether a state of \( B \) is reachable from a state of \( I \) by \( R \).
In a typical situation, \( S \) is the set of possible states of a program, \( R \) is the transition relation, \( I \) is the set of initial states and \( B \) is the set of bad states, to which we do not want to visit.

\begin{theorem}
    For any transition system \( (S, R) \) and sets \( I, B \subseteq S \) of states, the followinng are equivalent:
    \begin{itemize}
        \item \( (R^* I) \cap B = \emptyset \).
        \item \( I \cap \left((R^{\mathit{op}})^* B\right) = \emptyset\).
    \end{itemize}
\end{theorem}
\begin{proof}
    We prove that both conditions are equivalent to \( (R^* I) \cap \left((R^{\mathit{op}})^* B \right) = \emptyset \).
    \tk{to do}
    \qed
\end{proof}


Consider the following problem:
\begin{align*}
    & \forall i. & \varphi(i) &\Rightarrow P(i) \\
    & \forall x, y. & P(x) \wedge \rho(x,y) &\Rightarrow P(y) \\
    & \forall j. & P(j) &\Rightarrow \neg \psi(j). 
\end{align*}
The satisfiability problem for the above system is equivalent to the reachability problem where the initial state set is \( \{ s \mid \varphi(s) \} \), the transition relation is \( \{ (x,y) \mid \rho(x,y) \} \) and the bad state set is \( \{ s' \mid \psi(s') \} \). 

This problem can be solved by the following iterative computation (provided thet \( S \) is finite; the following observation is applicable to the case where \( S \) is infinite in a certain sense):
\begin{enumerate}
    \item Set \( X \leftarrow \{ i \mid \varphi(i) \} \).
    \item If \( X \cap \{ j \mid \psi(j) \} \neq \emptyset \) then return "UNSAT".
    \item If \( \{ y \mid \exists x \in X. R(x,y) \} \subseteq X \) then return "SAT".
    \item Set \( X \leftarrow X \cup \{ y \mid \exists x \in X. R(x,y) \} \).
    \item Goto 2.
\end{enumerate}
The invarint of the algorithm is that \( X \) is an under-approximation of the minimum solution of \( \{ \forall i. \varphi(i) \Rightarrow P(i),~ \forall x,y.P(x) \wedge \rho(x,y) \Rightarrow P(y) \} \).

The dual approach solves the same problem as follows.
The invarint is that the variable \( Y \) is an over-approximation of the greatest solution of \( \{ \forall x,y. P(x) \wedge \rho(x,y) \Rightarrow P(y),~ \forall j. P(j) \Rightarrow \neg \psi(j) \} \).
\begin{enumerate}
    \item Set \( Y \leftarrow \{ j \mid \neg \psi(j) \} \).
    \item If \( \{ i \mid \varphi(i) \} \setminus Y \neq \emptyset \) then return "UNSAT".
    \item If \( Y \cap \{ x \mid \exists y \in (S \setminus Y). R(x,y) \} = \emptyset \) then return "SAT".
    \item Set \( Y \leftarrow Y \setminus \{ x \mid \exists y \in (S \setminus Y). R(x,y) \} \).
    \item Goto 2.
\end{enumerate}

This algorithm can be made more understandable when one records the complement of \( Y \).
\begin{enumerate}
    \item Set \( \bar{Y} \leftarrow \{ j \mid \psi(j) \} \).
    \item If \( \bar{Y} \cap \{ i \mid \varphi(i) \} \neq \emptyset \) then return "UNSAT".
    \item If \( \{ x \mid \exists y \in \bar{Y}. R(x,y) \} \subseteq \bar{Y} \) then return "SAT".
    \item Set \( \bar{Y} \leftarrow \bar{Y} \cup \{ x \mid \exists y \in \bar{Y}. R(x,y) \} \).
    \item Goto 2.
\end{enumerate}
Actually this is the first algorithm for the \emph{dual} system:
\begin{align*}
    & \forall j. & \psi(j) &\Rightarrow \bar{P}(j) \\ 
    & \forall x, y. & \bar{P}(y) \wedge \rho(x,y) &\Rightarrow \bar{P}(x) \\
    & \forall i. & \bar{P}(i) &\Rightarrow \neg \varphi(i).
\end{align*}
The third algorithm calculate the reachable set from \( \psi(j) \), i.e.~the bad state set, via the transition relation \( \rho(x,y) \) by the opposite direction.

\subsection{The dual of linear CHC satisfiability}

\begin{theorem}
    Let \( A \) be a complete lattice and suppose that \( F(X) \le Y \) if and only if \( X \le G(Y) \) for every \( X \) and \( Y \) in \( A \).
    Then the following are equivalent:
    \begin{itemize}
        \item \( (\nu X. F(X) \sqcup I) \le B^{\bot} \).
        \item \( I \le (\nu Y. G(Y) \sqcap B^{\bot}) \).
    \end{itemize}
\end{theorem}
\begin{proof}
    We prove the both conditions are equivalent to \( (\nu X. F(X) \sqcup I) \le (\nu Y. G(Y) \sqcap B^{\bot}) \).
    This condition is obviously stronger than the above conditions.
    We prove \( (\nu X. F(X) \sqcup I) \le B^{\bot} \) implies \( (\nu X. F(X) \sqcup I) \le (\nu Y. G(Y) \sqcap B^{\bot}) \).
    Let \( \hat{G}(Y) := G(Y) \sqcup B^{\bot} \).
    Then \(\nu Y.G(Y) \sqcap B^{\bot} = \nu Y. \hat{G}(Y) \) is equvalent to
    \begin{equation*}
        \bigsqcap_{\alpha \colon \mathrm{Ordinal}} \hat{G}^\alpha(\top),
    \end{equation*}
    where \( \hat{G}^{\alpha+1}(Y) := \hat{G}(\hat{G}^{\alpha}(Y)) \) and, for a limit cardinal \( \beta \),
    \begin{equation*}
        \hat{G}^{\beta} := \bigsqcap_{\alpha < \beta} \hat{G}^\alpha(Y).
    \end{equation*}
    Hence it suffices to show that
    \begin{equation*}
        (\mu X. F(X) \sqcup I) \le \hat{G}^{\alpha}(\top)
    \end{equation*}
    for every ordinal \( \alpha \).
    We prove this claim by tnansfinite induction.
    The case that \( \alpha \) is a limit ordinal is trivial.
    Assume that \( \alpha = \beta + 1 \).
    By the induction hypothesis,
    \begin{equation*}
        (\mu X. F(X) \sqcup I) \le \hat{G}^{\beta}(\top).
    \end{equation*}
    Since
    \begin{equation*}
        F(\mu X. F(X) \sqcup I) \le F(\mu X. F(X) \sqcup I) \sqcup I = \mu X. F(X) \sqcup I,
    \end{equation*}
    we have
    \begin{equation*}
        F(\mu X. F(X) \sqcup I) \le \hat{G}^\beta(\top).
    \end{equation*}
    By the assumption, this is equivalent to
    \begin{equation*}
        \mu X. F(X) \sqcup I \le G(\hat{G}^\beta(\top)).
    \end{equation*}
    Since \( \mu X. F(X) \sqcup I \le B^{\bot} \) from the assumption, we have
    \begin{equation*}
        \mu X. F(X) \sqcup I \le G(\hat{G}^\beta(\top)) \sqcap B^{\bot} = \hat{G}(\hat{G}^\beta(\top)).
    \end{equation*}
    The proof of \( I \le (\nu Y. G(Y) \sqcap B^{\bot}) \) implies \( (\nu X. F(X) \sqcup I) \le (\nu Y. G(Y) \sqcap B^{\bot}) \) is similar.
    \qed
\end{proof}

Therefore one can prove \( I \le (\nu Y. G(Y) \sqcap B^{\bot}) \) instead of proving \( \mu X. F(X) \sqcup I \).
As we shall see, PDR can be seen as a proof search for the judgement \( I \vdash (\nu Y. G(Y) \sqcap B^{\bot}) \) corresponding to the former inequality.
In this sense, PDR solves the dual problem.

\begin{remark}
    Here is a gap between semantics and proofs, which should not be missed: the adjunction \( F \dashv G \), which can be written as \( F(X) \vdash Y \) if and only if \( X \vdash G(Y) \), should be \emph{provable}.
    That means, there should be a proof
    \begin{equation*}
        \dfrac{\dfrac{F(X) \vdash Y}{\vdots}}{X \vdash G(Y)}
    \end{equation*}
    in which there is a trace from \( G(Y) \) to \( Y \).
    \qed
\end{remark}

Given \( F : (S \to \Omega) \to (S \to \Omega) \), does there exist the adjoint \( G \)?
Unfortunately the following simple characterization gives the answer.
\begin{theorem}
    \( F : (S \to \Omega) \to (S \to \Omega) \) has a right adjoint if and only if \( F \) preserves joins, i.e.~\( F(\bigsqcup_{i \in I} x_i) = \bigsqcup_{i \in I} F(x_i) \).
    This condition is known as \emph{linearity}.
    In fact, there exists a relation \( R \subseteq S \times S \) such that
    \begin{equation*}
        F(X) = \{ y \in S \mid \exists x \in S. xRy \}.
    \end{equation*}
    So the direct application of the above argument does not go beyond the simplest case, namely, the reachability problem.
\end{theorem}
\begin{proof}
    Let \( R = \{ (x,y) \in S \times S \mid y \in F(\{x\}) \} \).
    It is not difficult to see that this relation \( R \) satisfies the above condition.
    \qed
\end{proof}



\subsection{The dual of general CHC satisfiability}
The general form of CHCs (with unique predicate variable) has the form:
\begin{align*}
    & \forall i. & \varphi(i) &\Rightarrow P(i) \\
    & \forall x_1,\dots,x_n, y. & P(x_1) \wedge \dots \wedge P(x_n) \wedge \rho(x_1,\dots,x_n,y) &\Rightarrow P(y) \\
    & \forall j. & P(j) &\Rightarrow \neg \psi(j). 
\end{align*}
The formal dual is of the form:
\begin{align*}
    & \forall j. & \psi(j) &\Rightarrow \bar{P}(j) \\ 
    & \forall x, y. & \bar{P}(y) \wedge \rho(x_1,\dots,x_n,y) &\Rightarrow \bar{P}(x_1) \vee \dots \vee \bar{P}(x_n) \\
    & \forall i. & \bar{P}(i) &\Rightarrow \neg \varphi(i).
\end{align*}
Unlike the case of the linear CHCs, the dual of a general CHC system is not a CHC system; there may be a disjunctive head.

The iterative algorithm is applicable to this non-CHC case as well, by allowing nondetermisism;
if one finds that \( \bar{P}(y) \) and \( \rho(x_1, \dots, x_n, y) \), the algorithm nondeterministically choose one element from \( x_1, \dots, x_n \) and add it to \( \bar{P} \).
\begin{enumerate}
    \item Set \( \bar{Y} \leftarrow \{ j \mid \psi(j) \} \).
    \item If \( \bar{Y} \cap \{ i \mid \varphi(i) \} \neq \emptyset \) then return "UNKNOWN".
    \item If \( \forall y \in \bar{Y}. \forall x_1, \dots, x_n. \rho(x_1,\dots,x_n,y) \Rightarrow \bar{Y} \cap \{ x_1, \dots, x_n \} \neq \emptyset \) then return "SAT".
    \item For each \( (x_1,\dots,x_n,y) \) such that \( y \in \bar{Y} \):
    \begin{enumerate}
        \item Nondeterministically choose \( x \leftarrow \{ x_1, \dots, x_n \} \).
        \item \( \bar{Y} \leftarrow \bar{Y} \cup \{x\} \).
    \end{enumerate}
    \item Goto 2.
\end{enumerate}
If the above "dual" system has a solution, then this algorithm has an execution path to "SAT" answer.

Furthermore one can determinise the above algorithm by a well-known general idea: we can record all possibilities by a set.
Hence we should now remember not just a set but a family of sets; and the algorithm returs "SAT" if there exists a set in the family that witnesses the satisfiability.
\begin{enumerate}
    \item Set \( \bar{\mathbb{Y}} \leftarrow \{ \{ j \mid \psi(j) \} \}\).
    \item For each \( \bar{Y} \in \bar{\mathbb{Y}} \):
    \begin{itemize}
        \item If \( \bar{Y} \cap \{ i \mid \varphi(i) \} \neq \emptyset \) then \( \bar{\mathbb{Y}} \leftarrow \bar{\mathbb{Y}} \setminus \{\bar{Y}\} \). 
    \end{itemize}
    \item If \( \bar{\mathbb{Y}} = \emptyset \) then return "UNSAT".
    \item For each \( \bar{Y} \in \bar{\mathbb{Y}} \):
    \begin{itemize}
        \item If \( \forall y \in \bar{Y}. \forall x_1, \dots, x_n. \rho(x_1,\dots,x_n,y) \Rightarrow \bar{Y} \cap \{ x_1, \dots, x_n \} \neq \emptyset \) then return "SAT".
    \end{itemize}
    \item Set \( \bar{\mathbb{Z}} \leftarrow \emptyset \).
    \item For each \( \bar{Y} \in \bar{\mathbb{Y}} \):
    \begin{enumerate}
        \item Set \( \bar{\mathbb{T}} \leftarrow \{ \bar{Y} \} \).
        \item For each \( (x_1,\dots,x_n,y) \) such that \( y \in \bar{Y} \):
        \begin{enumerate}
            \item Set \( \bar{\mathbb{T}} \leftarrow \{ \bar{T} \cup \{ x_i \} \mid \bar{T} \in \bar{\mathbb{T}}, 1 \le i \le n \} \).
        \end{enumerate}
        \item Set \( \bar{\mathbb{Z}} \leftarrow \bar{\mathbb{Z}} \cup \bar{\mathbb{T}} \).
    \end{enumerate}
    \item Set \( \bar{\mathbb{Y}} \leftarrow \bar{\mathbb{T}} \).
    \item Goto 2.
\end{enumerate}

Now the question is whether this process can be expressed as a fixed-point computation in a higher-order fixed-point logic.
It is indeed possible by slightly changing the algorithm:
instead of recording the above mentioned \( \bar{\mathbb{Y}} \), one can keep trace its over-approximations \( \{ \bar{Z} \mid \exists \bar{Y} \in \bar{\mathbb{Y}}. \bar{Y} \subseteq \bar{Z} \} \).
That means, we add the following statement between \( 7 \) and \( 8 \):
\begin{itemize}
    \item Set \( \bar{\mathbb{Y}} \leftarrow \{ \bar{Z} \mid \exists \bar{Y} \in \bar{\mathbb{Y}}. \bar{Y} \subseteq \bar{Z} \} \).
\end{itemize}
Then the above described update of \( \bar{\mathbb{Y}} \) in each round can be more concisely described as follows:
\begin{equation*}
    \mathcal{G}(\bar{\mathbb{Y}})(\bar{Y}) = \left[ \left\{ y \in \bar{Y} ~\middle|~ \forall x_1,\dots,x_n. \rho(x_1,\dots,x_n,y) \Rightarrow \bigvee_{1\le i \le n} x_i \in \bar{Y} \right\} \in \bar{\mathbb{Y}} \right]
\end{equation*}
\tk{Is this really true?}

As a consequence, the dual problem asks if
\begin{equation*}
    I^{\bot} \in \left(\nu \bar{\mathbb{Y}} \sqsupseteq B^{\uparrow}. \mathcal{G}(\bar{\mathbb{Y}}) \right).
\end{equation*}
where
\begin{align*}
    I^{\bot} &:= \{ i \in S \mid \neg \varphi(i) \} \\
    B &:= \{ j \mid \psi(j) \} \\
    B^{\uparrow} &:= \{ \bar{Z} \mid B \subseteq \bar{Z} \}.
\end{align*}

\tk{For this generation function \( \mathcal{G} \), do we have \( F(X) \in \mathbb{Y} \) iff \( X \in \mathcal{G}(\mathbb{Y}) \)?}

% \subsection{On fixed-points}
% Conisder the following problem.
% Let \( S \) be a set of \emph{states}.
% We have two subsets: \( I \subseteq S \) is the set of \emph{initial positions} and \( B \subseteq S \) is the set of \emph{bad positions}.
% We also have a relation \( R \subseteq S \times S \), describing the nondeterministic transition rule.
% We say that a state \( s \in S \) is \emph{reachable from} \( s_0 \in S \) if \( s_0 R^* s) \), where \( R^* \) is the transitive closure of \( R \).
% Let \( R^* I := \{ s \in S \mid \exists s_0 \in I. s_0 R^* s \} \).
% We would like to known whether \( R^* I \cap B = \emptyset \), i.e.~whether a bad state is reachable from an initial position.

% The problem can be described by uisg the fixed-point logic.
% Let \( F\colon \mathcal{P}(S) \to \mathcal{P}(S) \) be the following function:
% \begin{equation*}
%     F(X) ~:=~ \{ y \in S \mid \exists x \in X. x R y \}.
% \end{equation*}
% Let us write \( \mu X \ge I. F(X) \) for the least fixed-point of \( F \) subsuming \( I \), namely,
% \begin{equation*}
%     \mu X \ge I. F(X) ~:=~ \min \{ Y \subseteq S \mid F(Y) = Y \wedge Y \supseteq I \}.
% \end{equation*}
% (Note that the well-definedness of this notion itself is nontrivial.)
% Then
% \begin{equation*}
%     R^* I ~=~ \mu X \ge I. F(X).
% \end{equation*}
% So the problem is whether
% \begin{equation*}
%     (\mu X \ge I. F(X)) \cap B = \emptyset,
% \end{equation*}
% or equivalently,
% \begin{equation*}
%     (\mu X \ge I. F(X)) \subseteq B^\bot,
% \end{equation*}
% where \( B^\bot \) is the complement of \( B \).

% TODOOOOOOOOOOOOO!

% Suppose that all of \( I \), \( B \) and \( R \) are described by logical formulas, say \( \varphi_I \), \( \varphi_B \) and \( \varphi_R \).
% Then this can be seen as the validity problem of the following judgement:
% \begin{equation*}
%     \mu X \ge \varphi_I. \lambda y : S. \exists x. (x \in X) \wedge \varphi_R(x,y) ~\vdash~ \neg \varphi_B.
% \end{equation*}


% \subsection{Basics of fixed-points}
% Let \( S \) be a (po)set and \( \Omega = \{ \bot, \top \} \) be the two-valued Boolean algebra (as a poset).
% Then \( S \to \Omega \) is the set of properties on \( S \).

% Let \( F \colon (S \to \Omega) \to (S \to \Omega) \) be a predicate transformer.
% Intuitively \( F(I) \) is the subset of \( S \) reachable from \( I \) by one-step.
% We assume \( I \subseteq F(I) \) for simplicity.
% We should check whether this is really needed, anyway.

% Let \( \mu X \ge I. F(X) \) be the least fixed-point greater than \( I \).
% Let \( \check{F} \) and \( \hat{F} \) be the functions defined by
% \begin{align*}
%     \check{F}(X) &:= F(X) \sqcup X \\
%     \hat{F}(X) &:= F(X) \sqcap X.
% \end{align*}
% \begin{proposition}
%     If \( X \) is a fixed-point of \( F \), then so is \( \check{F} \) and \( \hat{F} \).
% \end{proposition}
% \begin{proof}
%     Assume that \( F(X) = X \).
%     Then \( \check{F}(X) = F(X) \sqcup X = X \sqcup X = X \).
%     Similarly \( \hat{F}(X) = F(X) \sqcap X = X \sqcap X = X \).
%     \qed
% \end{proof}

% Hence \( (\mu X \ge I. F(X)) = (\mu X \ge I. \check{F}(X)) \) and \( (\nu Y \le B^{\bot}. G(Y)) = (\nu Y \le B^{\bot}. \hat{G}(Y)) \).
% An important point is that \( \check{F}(X) \) is inflational, i.e.~\( \check{F}(X) \ge X \) for every \( X \).
% In this case, the least fixed-point subsuming \( I \) can be calculated by the (transfinitely many) iterative applications of \( \check{F} \) to \( I \):
% \begin{equation*}
%     (\mu X \ge I. \check{F}(X)) ~=~ \bigsqcup_{\alpha} \check{F}^\alpha(I).
% \end{equation*}

% One has
% \begin{equation*}
%     \mu X \ge I. F(X) = \bigsqcup_{\alpha \in \mathrm{ord}} \check{F}^{\alpha}(I)
% \end{equation*}
% where for a limit ordinal \( \alpha \), we define
% \begin{equation*}
%     \check{F}^{\alpha}(X) := \bigsqcup_{\beta < \alpha} \check{F}^\beta(X).
% \end{equation*}
% Similarly we define \( \check{F}_\alpha \) by
% \begin{equation*}
%     \check{F}_{\alpha}(X) := \sqcap_{\beta < \alpha} \check{F}_\beta(X).
% \end{equation*}
% \begin{theorem}
% Assume \( \check{F}(X) \le Y \Leftrightarrow X \le \hat{G}(Y) \).
% Then the following are equivalent:
% \begin{enumerate}
%     \item \( \mu X \ge I. F(X) \le B^{\bot} \).
%     \item \( \mu X \ge I. F(X) \le \nu Y \le B^{\bot}. G(Y) \).
%     \item \( I \le \nu Y \le B^{\bot}. G(Y) \).
% \end{enumerate}
% \end{theorem}
% \begin{proof}
% Obviously (2) implies (1) and (3).
% We prove that (1) implies (2).

% Assume that \( \mu X \ge I. F(X) \le B^{\bot} \).
% We prove \( \mu X \ge I. F(X) \le \hat{G}_\alpha(B^{\bot}) \) by induction on \( \alpha \).
% The case \(\alpha = 0 \) follows from the assumption.
% For \( \alpha = \beta +1 \), we have
% \begin{equation*}
%     \check{F}(\mu X \ge I. F(X)) = \mu X \ge I. F(X) \le \hat{G}_{\beta}(B^{\bot})
% \end{equation*}
% by the induction hypothesis.
% Since \( \check{F}(A) \le B \) if and only if \( A \le \hat{G}(B) \), one has
% \begin{equation*}
%     \mu X \ge I. F(X) \le \hat{G}(\hat{G}_{\beta}(B^{\bot})) = \hat{G}_{\beta+1}(B^{\bot})
% \end{equation*}
% For the case \( \alpha \) being a limit ordinal, we have
% \begin{equation*}
%     \mu X \ge I. F(X) \le \hat{G}_{\beta}(B^\bot)
% \end{equation*}
% for every \( \beta < \alpha \) by the induction hypothesis.
% Hence
% \begin{equation*}
%     \mu X \ge I. F(X) \le \sqcap_{\beta < \alpha} \hat{G}_{\beta}(B^\bot) = \hat{G}_\alpha(B^\bot).
% \end{equation*}
% \qed
% \end{proof}

% \begin{lemma}
%     Assume \( F(X) \le Y \) if and only if \( X \le G(Y) \).
%     Then \( \check{F}(X) \le Y \) if and only if \( X \le \hat{G}(Y) \).
% \end{lemma}
% \begin{proof}
%     The former condition is equivalent to \( X \le Y \) and \( F(X) \le Y \) since \( \check{F}(X) = X \sqcup F(X) \).
%     The latter condition is equivalent to \( X \le Y \) and \( X \le \hat{G}(Y) \).  Hence, by the assumption, these conditions coincide.
% \qed
% \end{proof}


% \begin{theorem}
%     Suppose \( F \dashv G \).
%     Then the following conditions are equivalest:
%     \begin{enumerate}
%         \item \( (\mu X \ge I. F(X)) \subseteq B^{\bot} \)
%         \item \( (\mu X \ge I. F(X)) \subseteq (\nu Y \le B^{\bot}. G(Y)) \)
%         \item \( I \subseteq (\nu Y \le B^{\bot}. G(Y)) \).
%     \end{enumerate}
% \end{theorem}


\subsection{On cyclic proofs}



